Interventional Bag Multi-Instance Learning On Whole-Slide Pathological Images

Multi-instance learning (MIL) is an effective paradigm for whole-slide pathological images (WSIs) classification to handle the gigapixel resolution and slide-level label. Prevailing MIL methods primarily focus on improving the feature extractor and aggregator. However, one deficiency of these methods is that the bag contextual prior may trick the model into capturing spurious correlations between bags and labels. This deficiency is a confounder that limits the performance of existing MIL methods. In this paper, we propose a novel scheme, Interventional Bag Multi-Instance Learning (IBMIL), to achieve deconfounded bag-level prediction. Unlike traditional likelihood-based strategies, the proposed scheme is based on the backdoor adjustment to achieve the interventional training, thus is capable of suppressing the bias caused by the bag contextual prior. Note that the principle of IBMIL is orthogonal to existing bag MIL methods. Therefore, IBMIL is able to bring consistent performance boosting to existing schemes, achieving new state-of-the-art performance. Code is available at https://github.com/HHHedo/IBMIL.

==> algorithms/stage3.tex <==
% \begin{algorithm} 
% 	\caption{Pseudocode of Interventional Training} 
% 	\label{alg3} 
% 	\begin{algorithmic}
% 		\REQUIRE $n \geq 0 \vee x \neq 0$ 
% 		\ENSURE $y = x^n$ 
% 		\STATE $y \gets 1$ 
% 		\IF{$n < 0$} 
% 		\STATE $X \gets 1 / x$ 
% 		\STATE $N \gets -n$ 
% 		\ELSE 
% 		\STATE $X \gets x$ 
% 		\STATE $N \gets n$ 
% 		\ENDIF 
% 		\WHILE{$N \neq 0$} 
% 		\IF{$N$ is even} 
% 		\STATE $X \gets X \times X$ 
% 		\STATE $N \gets N / 2$ 
% 		\ELSE[$N$ is odd] \STATE $y \gets y \times X$ 
% 		\STATE $N \gets N - 1$ 
% 		\ENDIF 
% 		\ENDWHILE 
% 	\end{algorithmic} 
% \end{algorithm}
% A bag feature B with shape (1, d) generated by aggregator,

\begin{algorithm} 
	\caption{Pseudocode of Interventional Training} 
	\label{alg3} 
    \definecolor{codeblue}{rgb}{0.25,0.5,0.5}
    \definecolor{codekw}{rgb}{0.85, 0.18, 0.50}
    \lstset{
      backgroundcolor=\color{white},
      basicstyle=\fontsize{7.5pt}{7.5pt}\ttfamily\selectfont,
      columns=fullflexible,
      breaklines=true,
      captionpos=b,
      commentstyle=\fontsize{7.5pt}{7.5pt}\color{codeblue},
      keywordstyle=\fontsize{7.5pt}{7.5pt}\color{codekw},
    }
    \begin{lstlisting}[language=python]
    # Inputs: 
    # Confounder dictionary C with shape (K, d),
    # Features of instances [b_1, ..., b_n], each with shape (1, d)
    # Ground truth Y
    
    # Outputs: 
    # Bag level prediction Y_hat, Loss L for optimizing network parameters  
    
    # Previous MIL training: 
    B = aggregator_network([b_1, ..., b_n]) # B is the bag feature with shape (1, d)
    Y_hat = classify_head(B)
    L = criterion(Y_hat, Y)
    
    # Interventional training: 
    B = aggregator_network([b_1, ..., b_n]) # B is the bag feature with shape (1, d)
    B_q = linear1(B) # Projection matrix W_1, B_q with shape (1, l)
    
    C.requires_grad = False # freeze C
    C_k = linear2(C) # Projection matrix W_2, C_k with shape (K, l)
    
    Alpha = torch.mm(C_k, B_q.T) 
    Alpha = F.softmax(Alpha / sqrt(l), dim=0) # Normalize weighted scores
    C_ave = torch.mm(Alpha.T, C) # Weighted average, C_ave with shape (1, d)
    
    B = torch.cat([B, C_ave], dim=1)
    Y_hat = classify_head(B)
    L = criterion(Y_hat, Y)
    
    \end{lstlisting}
\end{algorithm}

==> figs/confounder.tex <==
\begin{figure}[t]
	\centering
	\begin{minipage}{1.0\linewidth}
	
	\centering
	\begin{minipage}{0.48\linewidth}
		\centering
		\includegraphics[width=0.93\linewidth]{figs/cls_spec.pdf}
		\subcaption{}
		\label{ab:cls_spec}%文中引用该图片代号
	\end{minipage}
	\begin{minipage}{0.48\linewidth}
		\centering
		\includegraphics[width=0.93\linewidth]{figs/merge.pdf}
		\subcaption{}
		\label{ab:merge}%文中引用该图片代号
	\end{minipage}
	
	%\qquad
	%让图片换行，
	
	\end{minipage}
	
	
	\caption{Analysis of constitution of confounder set. (a) Class-specific vs. class-agnostic. (b) Confounder set from TCGA vs. TCGA+Camelyon16.}
\end{figure}

==> figs/total_ab_part1.tex <==
\begin{figure}[htb]
	\centering
	\begin{minipage}{1.0\linewidth}
	
	\centering
	\begin{minipage}{0.48\linewidth}
		\centering
		\includegraphics[width=0.93\linewidth]{figs/num_K.pdf}
		\subcaption{}
		\label{ab:dic size}%文中引用该图片代号
	\end{minipage}
	\begin{minipage}{0.48\linewidth}
		\centering
		\includegraphics[width=0.93\linewidth]{figs/num_dim.pdf}
		\subcaption{}
		\label{ab: feat dim}%文中引用该图片代号
	\end{minipage}
	
	%\qquad
	%让图片换行，
	
	\end{minipage}
	
	
	\caption{Ablation studies of (a) Size of confounder dictionary, and (b) Dimension of joint feature space.}
\end{figure}

==> figs/total_ab_part2.tex <==
\begin{figure}[htb]
	\centering
	\begin{minipage}{1.0\linewidth}
	
	\centering
	\begin{minipage}{0.48\linewidth}
		\centering
		\includegraphics[width=0.93\linewidth]{figs/epoch.pdf}
		\subcaption{}
		\label{ab: epoch}%文中引用该图片代号
	\end{minipage}
	\begin{minipage}{0.48\linewidth}
		\centering
		%\includegraphics[width=0.93\linewidth]{figs/cls_spec.pdf}
		\includegraphics[width=0.93\linewidth]{figs/nopara.pdf}
		\subcaption{}
	\label{ab: nopara}%文中引用该图片代号
	
	\end{minipage}
	%\qquad
	%让图片换行，
	
	\end{minipage}
	
	
	\caption{Analysis of (a) More training epochs of baselines, and (b) Constitution of confounder set. Experiments are conducted on TCGA-NSCLC dataset.
	We choose ResNet-18 as the feature extractor in (a) and ABMIL as the aggregator in (b). }
\end{figure}

==> tables/R_reportedVSori.tex <==

\begin{table}[t]
\caption{Main results (\%) on Camelyon16 and TCGA-NSCLC. }
\centering
% \resizebox{1\textwidth}{!}
{\begin{tabular}{clccccccccc} 
\toprule
\multicolumn{3}{c}{\multirow{2}{*}{\diagbox[width=12em]{\textbf{Method}}{\textbf{Performance}}}} & \multicolumn{4}{c}{Camelyon16} & \multicolumn{4}{c}{TCGA-NSCLC} \\ 
\cmidrule(lr){4-7}  
\cmidrule(lr){8-11} 
\multicolumn{3}{r}{} & Precision & Recall  & Accuracy & AUC & Precision & Recall  & Accuracy & AUC\\

% ####################
\hline
\multirow{12}{*}{\rotatebox{90}{\makecell{CTransPath \\ SRCL}}}
&\multirow{3}{*}{ABMIL}&Reported&91.84&	89.09&	90.70&	92.33
&90.76	&90.40&	90.48&	95.87 \\

&&\cite{li2021dual}& 95.29&	92.31&	84.50&	86.53 & 91.92&	91.93&	90.00&	94.88 \\ 

\cline{2-11}  
&\multirow{3}{*}{DSMIL}&Reported& 89.24&	88.10&	89.15&	93.26&
92.11&	92.79&	90.95&	97.13\\
&&\cite{li2021dual} & 91.05&	91.30&	86.82&	89.44 
&92.05&	93.82&	91.90&	95.83 \\ 

\cline{2-11}  
&\multirow{3}{*}{TransMIL}&& 95.83&	93.27&	94.57&	95.88 &92.05&	93.82&	91.90&	95.55\\

&&+IBMIL &96.48&	95.50&	96.12&	97.00 &93.94&	93.76&	93.81&	97.24\\ 

\cline{2-11}  
&\multirow{3}{*}{\makecell{DTFD-MIL \\(MaxS) } }&& 95.87&	94.54&	95.35&	96.18&
90.41&	88.40&	88.57&	94.88\\

&&+IBMIL & 96.95	&95.19&	96.12&	96.28 
&91.17&	90.89&	90.95&	96.57 \\ 

\bottomrule  
\end{tabular}

\label{tab:RVSO}
}
\end{table}

==> tables/ab_K.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table}[htbp]
% \caption{Comparisons of different number of confounders. }
% \label{tab:ab_imple}
% \centering
% \resizebox{0.75\linewidth}{!}{
% \begin{tabular}{cccccc}
% \toprule
% Dataset                   & $K$        & Precision   & Recall   & Accuracy   & AUC  \\ \hline
% \multirow{4}{*}{\rotatebox{90}{\makecell{Camelyon \\ 16 }}} 
%                       & 2        & 88.58 & 87.14 & 88.37 & 90.43 \\
%                       & 4        & 87.30 & 85.21 & 86.82 & 89.44 \\
%                       & 8        & 88.06 & 82.36 & 85.27 & 87.96 \\
%                       & 16       & 86.25 & 84.57 & 86.05 & 88.41 \\ 
% \midrule
% \multirow{4}{*}{\rotatebox{90}{\makecell{TCGA- \\ NSCLC }}}  

%                       & 2        & 85.19 & 83.66 & 83.81 & 91.57 \\
%                       & 4        & 83.89 & 83.66 & 83.81 & 91.57 \\
%                       & 8        & 85.42 & 85.17 & 85.24 & 91.26 \\
%                       & 16       & 84.82 & 84.72 & 84.76 & 91.69 \\ 
                      
% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[htbp]
\caption{Comparison of different size of confounder dictionary. }
%Experiments are conducted on TCGA-NSCLC dataset and ABMIL method applied with our proposed IBML.}
\label{tab:ab_K}
\centering
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
\makecell{Feature \\ Extractor}                    & $K$        & Precision   & Recall   & Accuracy   & AUC  \\ \hline
\multirow{4}{*} {ResNet}
%{\rotatebox{90}{\makecell{ResNet}}} 
                      & 2        & 85.19 & 83.66 & 83.81 & 91.57 \\
                      & 4        & 83.89 & 83.66 & 83.81 & 91.57 \\
                      & 8        & 85.42 & 85.17 & 85.24 & 91.26 \\
                      & 16       & 84.82 & 84.72 & 84.76 & 91.69 \\ 
\midrule
\multirow{4}{*}{CTrans}
%{\rotatebox{90}{\makecell{CTrans}}}  

                      & 2        & 90.47 &	90.47&	90.48 &	95.83 \\
                      & 4        & 91.43 &	91.43 &	91.43 &	96.66 \\
                      & 8        & 91.92  &	91.93&	91.90&	96.91 \\
                      & 16       & 91.09 &	91.01&	90.95&	96.55 \\ 
\midrule
\multirow{4}{*}{ViT}
%{\rotatebox{90}{\makecell{ViT}}}  

                      & 2        & 89.01 &	86.83&	88.37&	91.38 \\
                      & 4        & 89.01 &	86.83&	88.37&	91.36 \\
                      & 8        & 87.94 &	86.18&	87.60&	91.31 \\
                      & 16       & 89.01 &	86.83&	88.37&	91.41 \\ 
                      
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ab_dim.tex <==
\begin{table}[htbp]
\caption{Comparison  of different dimensions of joint feature space. }
%Experiments are conducted on TCGA-NSCLC dataset and ABMIL method applied with our proposed IBML. }
\label{tab:ab_dim}
\centering
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
Dim.                    & Precision   & Recall   & Accuracy   & AUC  \\ \hline
64  & 84.23 & 84.85 & 83.81 & 90.22 \\
 128                            & 85.42 & 85.17 & 85.24 & 91.26 \\
   256                          & 85.25 & 88.08 & 84.76 & 92.56 \\
      512                          & 84.41 & 84.34 & 84.29 & 90.68 \\


\bottomrule
\end{tabular}
}
\end{table}

==> tables/ab_freeze.tex <==
% \begin{table}[htbp]
% \caption{Impact of freezing confounders for different epochs from the start.} %Experiments are conducted on TCGA-NSCLC dataset and ABMIL method applied with our proposed IBML. }
% \label{tab:ab_freeze}
% \centering
% \resizebox{0.8\linewidth}{!}{
% \begin{tabular}{ccccc}
% \toprule
%                     & Precision   & Recall   & Accuracy   & AUC  \\ \hline
% 0  & 83.81 & 83.82 & 83.81  & 90.82 \\
%  5                            & 84.57 & 84.20 & 84.29 & 91.28 \\
%   10                          & 84.99 & 84.68  & 84.76 & 91.28  \\
%       $ \sim $end                         & 85.42 & 85.17 & 85.24 & 91.26  \\


% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{table}[t]
\caption{Comparison of learnable and unlearnable confounders.} %Experiments are conducted on TCGA-NSCLC dataset and ABMIL method applied with our proposed IBML. }
\label{tab:ab_freeze}
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
  Learnable                   & Precision   & Recall   & Accuracy   & AUC  \\ \hline
yes  & 83.81 & 83.82 & 83.81  & 90.82 \\
     no                      & 85.42 & 85.17 & 85.24 & 91.26  \\


\bottomrule
\end{tabular}
}
\end{table}

==> tables/ab_imple.tex <==
\begin{table}[t]
\caption{Comparison of different implementations of back-door adjustment. }
%Experiments are conducted on TCGA-NSCLC dataset and ABMIL method applied with our proposed IBML.}
\label{tab:ab_imple}
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
Method                    & Precision   & Recall   & Accuracy   & AUC  \\ \hline
$\oplus$  & 85.42 & 85.17 & 85.24 & 91.26 \\
 +                            & 84.99 & 84.68 & 84.76 & 89.28 \\
   -                          &84.70 & 84.18 &84.29 & 90.14 \\


\bottomrule
\end{tabular}
}
\end{table}

==> tables/ab_time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
\caption{Comparison of different training epochs of baseline methods. Experiments are conducted on TCGA-NSCLC dataset with feature extractor of ResNet-18.}
\label{tab:ab_time}
\centering
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{lccccc}
\toprule
Method                   & Epoch        & Precision   & Recall   & Accuracy   & AUC  \\ \hline
\multirow{2}{*}{ABMIL} 
                      & 50        & 82.75 &85.84 & 81.43 & 88.95 \\
                      & 100        & 82.77 & 83.00 & 81.90 & 88.25 \\
\midrule

\multirow{2}{*}{DSMIL} 
                      & 50        & 80.56 & 85.78 & 77.62 & 86.88 \\
                      & 100        & 79.46 & 84.9 & 74.76 & 86.31 \\

\midrule

\multirow{2}{*}{DTFD-MIL} 
                      & 50        & 88.11 & 88.12 & 88.10 & 92.36 \\
                      & 100        & 85.29 & 85.28 & 85.24 & 90.72 \\

\midrule

\multirow{2}{*}{TransMIL} 
                      & 50        & 85.46 & 85.31 & 85.24 & 90.70 \\
                      & 100        & 83.67 & 89.59 & 82.38 & 88.30 \\

                      
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ana_cls.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htbp]
\caption{Comparison of different choices of confounder set constitution. We build IBML upon ABMIL method and conduct experiments on various datasets and feature extractors.}
\label{tab:ana_cls}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\makecell{Feature \\ Extractor}                   & Dataset  &  \makecell{Class \\ Agnostic}     & Precision   & Recall   & Accuracy   & AUC  \\ \hline
\multirow{4}{*}{ResNet} & \multirow{2}{*}{C16}    & no    & 82.60 &	81.66 &	82.95 &	86.36  \\
                      &    & yes  & 88.06	&82.36&	85.27&	87.96  \\
                      & \multirow{2}{*}{TCGA }  & no     & 83.87 &	83.77& 	83.81 &	91.01  \\
                      &    & yes     & 85.42 &	85.17&	85.24&	91.26  \\
\midrule

\multirow{4}{*}{CTrans} & \multirow{2}{*}{C16}    & no    & 95.83 &	93.27 &	94.57 &	94.31 \\
                      &    & yes    & 95.29 &	92.31&	93.8&	93.83 \\
                      & \multirow{2}{*}{TCGA }  & no     & 93.43 &	93.39 &	93.33 &	97.06  \\
                      &  &  yes     &  92.38&	92.40&	92.38&	96.82  \\
\midrule

\multirow{4}{*}{ViT} & \multirow{2}{*}{C16}    & no    & 82.63&84.83&81.90&90.22 \\
                      &    & yes    & 87.94 &	86.18 &	87.60 &	91.31   \\
                      & \multirow{2}{*}{TCGA }  & no     & 90.11 &	89.41 &	89.52 &	92.95 \\
                      &   & yes     &  89.38 &	88.96 &	89.05 &	93.27  \\


                     
\bottomrule
\end{tabular}
}
\end{table}

==> tables/ana_conf.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
\begin{table}[t]
\caption{Comparison of different settings of constituting the confounder dictionary. }
\label{tab:ana_conf}
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
Method  & $C$ & Precision   & Recall   & Accuracy   & AUC  \\ 
\hline
\multirow{5}{*}{ABMIL} & /    & \color{gray}{82.75} & \color{gray}{85.84} & \color{gray}{81.43} & \color{gray}{88.95} \\
                        & Default & 84.82 &	84.72 &	84.76 &	91.69 \\
                      & Max        & 85.66 & 82.40 & 82.38 & 91.37 \\
                      & Mean        & 88.10 & 88.08 & 88.10 & 92.51 \\
                      & Instance        & 86.25 & 86.23 & 86.19 & 91.74 \\
\midrule

\multirow{5}{*}{DSMIL}  & /        & \color{gray}{80.56} & \color{gray}{85.78} & \color{gray}{77.62} & \color{gray}{86.88} \\
                        & Default & 81.54 &	83.39 &	78.10	 & 86.91 \\
                      & Max        & 79.62 &87.09 & 77.62 & 87.83 \\
                      & Mean        & 79.21 & 87.13 & 77.14 & 88.57 \\
                      & Instance        & 81.67 & 82.44 & 78.10 & 87.44 \\

                     
\bottomrule
\end{tabular}
}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[t]
% \caption{Comparison of different settings of constituting the confounder dictionary. }
% \label{tab:ana_conf}
% \centering
% \resizebox{0.9\linewidth}{!}{
% \begin{tabular}{cccccccccccc}
% \toprule
% Method  & Confounder & Precision   & Recall   & Accuracy   & AUC &Method  & Confounder & Precision   & Recall   & Accuracy   & AUC  \\ 
% \hline
% \multirow{5}{*}{\rotatebox{90}{ABMIL}} & /   & \color{gray}{82.75} & \color{gray}{85.84} & \color{gray}{81.43} & \color{gray}{88.95} & \multirow{5}{*}{\rotatebox{90}{DSMIL}} & /        & \color{gray}{80.56} & \color{gray}{85.78} & \color{gray}{77.62} & \color{gray}{86.88}\\
% & Default & 84.82 &	84.72 &	84.76 &	91.69 & & Default & 81.54 &	83.39 &	78.10	 & 86.91\\
% & Max  & 85.66 & 82.40 & 82.38 & 91.37 & & Max        & 79.62 &87.09 & 77.62 & 87.83\\
% & Mean        & 88.10 & 88.08 & 88.10 & 92.51 & & Mean        & 79.21 & 87.13 & 77.14 & 88.57 \\
% & Instance        & 86.25 & 86.23 & 86.19 & 91.74 & & Instance        & 81.67 & 82.44 & 78.10 & 87.44 \\    
% \bottomrule
% \end{tabular}
% }
% \end{table*}

==> tables/ana_knn.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Performance of KNN evaluation. }
\label{tab:ana_knn}
\centering
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{ccccc}
\toprule
\makecell{Feature \\ Extractor}                   & $K$       & Top 1   & Top 3   & Top 5    \\ \hline
\multirow{4}{*}{ResNet} & 2       & 82.38 & 71.42  &  /  \\
                      & 4       &80.00& 80.48 & 71.90   \\
                      & 8       & 81.90 & 80.48 & 80.48   \\
                      & 16       & 68.10 & 79.52 & 76.19   \\
\midrule

\multirow{4}{*}{CTrans} & 2       & 90.00 & 90.48 & /   \\
                      & 4       & 90.48 & 88.57 & 89.05   \\
                      & 8       & 90.48 & 90.48  & 89.05   \\
                      & 16       & 90.48 & 89.52 &  90.00  \\
                      
\midrule

\multirow{4}{*}{ViT} & 2       & 89.04 & 89.04  & /   \\
                      & 4       &  87.62& 88.10 & 88.57  \\
                      & 8       & 88.10 & 88.10 & 88.10   \\
                      & 16       &  88.10& 89.05  & 88.57   \\


                     
\bottomrule
\end{tabular}
}
\end{table}

% \begin{table}[t]
% \caption{Performance of KNN evaluation. }
% \label{tab:ana_knn}
% \centering
% \resizebox{0.65\linewidth}{!}{
% \begin{tabular}{ccccccc}
% \toprule
% \makecell{Feature \\ Extractor}                   & $K$       & Top 1   & Top 3   & K & Top 1 & Top 3    \\ \hline
% \multirow{2}{*}{ResNet} & 2       & 82.38 & 71.42  & 4 & 80.00& 80.48  \\
%                       & 8       &81.90 & 80.48 & 16 &68.10 & 79.52  \\

% \midrule

% \multirow{2}{*}{CTrans} & 2       & 90.00 & 90.48 & 4 & 90.48 & 88.57   \\
%                       & 8       & 90.48 & 90.48 & 16 & 90.48 & 89.52   \\

                      
% \midrule

% \multirow{2}{*}{ViT} & 2       & 89.04 & 89.04  & /   \\
%                       & 4       &  87.62& 88.10 & 88.57  \\
%                       & 8       & 88.10 & 88.10 & 88.10   \\
%                       & 16       &  88.10& 89.05  & 88.57   \\


                     
% \bottomrule
% \end{tabular}
% }
% \end{table}

==> tables/finetune.tex <==
\begin{table*}
\begin{center}
\setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \begin{tabular}{clcccccccc}
    \hline
        Decoder & Method & IIIT5K & IC03 & IC13 & SVT & IC15 & SVTP & CUTE80 & Avg\\ \hline
        \multirow{5}{*}{Atten} & Supervised baseline & 84.40 & 91.81 & 89.16 & 83.62 & 68.05 & 73.33 & 71.08 & 80.21 \\ 
        ~ & SeqCLR & 82.90 & 92.20 & 87.90 & - & - & - & - & -\\ 
        ~ & PerSec-CNN & 84.20 & - & 88.90 & 82.40 & 68.20 & 73.60 & 68.40 & -\\ 
        ~ & SeqMoCo & 84.40  & 92.73  & 89.85  & 84.54  & 69.30  & 74.88  & 64.81  & 80.08\\ 
        ~ & RCLSTR(Ours) & 86.03  & 92.73  & 91.13  & 83.15  & 69.15  & 74.88  & 67.94 & 80.72 \\ \hline
    \end{tabular}
\caption{\textbf{Fine-tuning results.} Accuracy of fine-tuning a pretrained model with labeled data. }
\label{tab:finetune}
\end{center}
\end{table*}

==> tables/gray_temp.tex <==
\begin{table*}[t]
	\subfloat[{Training Objective $\mathcal{L}$} \label{table:loss}]{
		\tablestyle{7pt}{1.05}
		\begin{tabular}{|ccc||c|}\thickhline
			\rowcolor{mygray}
			$\mathcal{L}_{\text{CE}}$ & $\mathcal{L}_{\text{PPC}}$ & $\mathcal{L}_{\text{PPD}}$  & mIoU  \\
			\rowcolor{mygray}
			(Eq.~\ref{eq:nce}) & 	(Eq.~\ref{eq:ppc}) & 	(Eq.~\ref{eq:ppd})  & (\%) \\ \hline\hline
			\cmark & &                    	 & 45.0\\
			\cmark &\cmark &          	&  45.9 \\
			\cmark & &\cmark           	&  45.4\\
			\cmark & \cmark&\cmark & 46.4\\
			\hline
		\end{tabular}
		%}
	}\hfill
	%	
	\subfloat[{Prototype Number $K$}\label{table:prototypenumber}]{%
		%\resizebox{0.23\textwidth}{!}{
		\tablestyle{5pt}{1.05}
		\begin{tabular}{|l||c|}\thickhline
			\rowcolor{mygray}
			\# Prototype & mIoU (\%)\\ \hline\hline
			~~~$K=1$  & 45.5 \\
			~~~$K=5$  & 46.0 \\
			~~~$K=10$  & 46.4 \\
			~~~$K=20$  & 46.5\\
			~~~$K=50$  & 46.4\\
			\hline
		\end{tabular}
		%}
	}\hfill
	%
	\subfloat[{Momentum Coefficient $\mu$}\label{table:momentum}]{%
		%\resizebox{0.23\textwidth}{!}{
		\tablestyle{6pt}{1.05}
		\begin{tabular}{|l||c|}\thickhline
			\rowcolor{mygray}
			Coefficient $\mu$ & mIoU (\%) \\\hline\hline
			~~$\mu=0$ & 44.9 \\
			~~$\mu=0.9$ & 45.9 \\
			~~$\mu=0.99$ & 46.0 \\
			~~$\mu=0.999$ & 46.4 \\
			~~$\mu=0.9999$ & 46.3 \\
			\hline
		\end{tabular}
		%	}
	}\hfill
	%
	\subfloat[{Distance Measure}\label{table:distance}]{%
		\tablestyle{8pt}{1.05}
		%\resizebox{0.20\textwidth}{!}{
		\begin{tabular}{|c||c|}\thickhline
			\rowcolor{mygray}
			Distance Measure & mIoU (\%) \\ \hline\hline
			Standard & 45.7\\
			Huberized & 45.2 \\
			Cosine  & 46.4 \\
			
			\hline
			\multicolumn{2}{c}{} \\
			\multicolumn{2}{c}{}
		\end{tabular}
		%	}
	}\hfill
	\vspace{-3pt}
	\captionsetup{font=small}
	\caption{\small A set of \textbf{ablative studies} (\S\ref{sec:ablation}) on ADE20K~\cite{zhou2017scene} \texttt{val}. All model variants use MiT-B2~\cite{xie2021segformer} as the backbone.}
	\label{tab:ablations}\vspace{-5mm}
\end{table*}

==> tables/hierarchical.tex <==
\begin{table*}[htb]
\begin{center}
    \centering
    \begin{tabular}{ccccccccc}
    \hline
         Hierarchies& IIIT5K & IC03 & IC13 & SVT & IC15 & SVTP & CUTE80 & Avg \\ \hline
         w/ subword \& word \& frame & 58.80 & 68.51 & 66.21 & 47.45 & 37.65 & 37.36 & 39.24 & 50.75\\ 
         w/ subword \& word & 56.30 & 66.90 & 64.63 & 43.59 & 35.19 & 35.50 & 35.07 & 48.17\\ 
         w/ subword \& frame & 50.07 & 62.17 & 58.82 & 36.01 & 30.52 & 27.29 & 28.82 & 41.96\\ \hline
    \end{tabular}
\caption{\textbf{Ablation of hierarchical relation module.} ``Hierarchies" represents different combinations of hierarchies for contrastive learning. All results are on representation qualities (decoder evaluation accuracy).}
\label{tab:hierarchical}
\end{center}
\begin{center}
\setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \begin{tabular}{ccccccccc}
    \hline
        Consistency & IIIT5K & IC03 & IC13 & SVT & IC15 & SVTP & CUTE80 & Avg\\ \hline
         w/ subword-word \& frame-subword & 60.83 & 75.20 & 69.66 & 51.78 & 41.12 & 44.03 & 39.93 & 54.65\\ 
         w/ subword-word & 59.47 & 70.24 & 66.60 & 47.30 & 36.11 & 38.14 & 32.29 & 50.02\\ 
         w/ frame-subword & 60.73 & 72.78 & 69.85 & 51.78 & 39.53 & 40.31 & 38.19 & 53.31\\ \hline
    \end{tabular}
\caption{\textbf{Ablation of relational consistency module.} Different kinds of consistency constraints are imposed separately to explore the effect of each constraint. All results are on representation qualities (decoder evaluation accuracy).}
\label{tab:consistency}
\end{center}
\end{table*}

==> tables/nokl.tex <==
\begin{table*}
\begin{center}
\setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \begin{tabular}{clccccccc}
    \hline
        Decoder & Method & IIIT5K & IC03 & IC13 & SVT & IC15 & SVTP & CUTE80 \\ \hline
        \multirow{4}{*}{Atten} & SeqMoCo & 50.97 & 58.36 & 55.86 & 35.55 & 29.42 & 28.53 & 30.56 \\ 
        ~ & SeqMoCo w/ reg & 56.80 & 68.74 & 64.04 & 44.36 & 35.77 & 36.43 & 37.15 \\ 
        ~ & SeqMoCo w/ reg \& hier & 61.33 & 72.32 & 67.29 & 49.15 & 38.04 & 41.55 & 37.50 \\ 
        ~ & SeqMoCo w/ reg \& hier \& con & 60.87 & 73.24 & 69.06 & 51.31 & 39.87 & 41.55 & 36.81 \\ \hline
    \end{tabular}
\caption{\textbf{Results without KL loss.} Ablation studies of module effect without KL loss.  Based on SeqMoCo, we compare our method with different modules, where "reg" denotes the regularization module, "hier" denotes the hierarchical module and "con" denotes the hierarchical consistency module. All results are on representation qualities (decoder evaluation accuracy).}
\label{tab:nokl}
\end{center}
\end{table*}

==> tables/non-para-agg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
Agg                    & Confounder            & K  & Precision & Recall & Accuracy & AUC   \\ \hline
\multirow{7}{*}{ABMIL} & -              & -  & 82.75     & 85.84  & 81.43    & 88.95 \\
                       & \multirow{2}{*}{Max}  & 2  & 85.16     & 84.77  & 84.76    & 91.72 \\
                       &                       & 4  & 83.76     & 85.3   & 83.33    & 91.77 \\ \cline{2-7}
                       & \multirow{4}{*}{Mean} & 2  & 85.71     & 85.71  & 85.71    & 91.67 \\
                       &                       & 4  & 83.92     & 84.33  & 83.81    & 91.19 \\
                       &                       & 8  & 86.77     & 87.18  & 86.67    & 92.35 \\
                       &                       & 16 & 88.10     & 88.08  & 88.10    & 92.51 \\
\midrule
\multirow{7}{*}{DSMIL} & -              & - & 80.56     & 85.78  & 77.62    & 86.88 \\
                       & \multirow{2}{*}{Max}  & 2  & 79.22     & 85.21  & 77.14    & 88.29 \\
                       &                       & 4  & 84.40     & 82.38  & 80.00    & 89.14 \\ \cline{2-7}
                       & \multirow{4}{*}{Mean} & 2  & 80.72     & 85.73  & 77.14    & 88.37 \\
                       &                       & 4  & 81.90     & 83.84  & 79.05    & 87.43 \\
                       &                       & 8  & 78.16     & 85.24  & 75.71    & 87.78 \\
                       &                       & 16 & 79.21     & 87.13  & 77.14    & 88.57\\
\bottomrule
\end{tabular}
}

\end{table}

==> tables/non-para.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\resizebox{0.75\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule
Agg                   & K        & Precision   & Recall   & Accuracy   & AUC  \\ \hline
\multirow{5}{*}{Mean} & - & 77.13 & 71.60 & 71.43 & 80.68 \\
                      & 2        & 81.97 & 81.49 & 81.43 & 85.81 \\
                      & 4        & 82.04 & 81.56 & 81.43 & 87.10 \\
                      & 8        & 84.50 & 80.46 & 80.48 & 89.14 \\
                      & 16       & 85.13 & 78.16 & 78.10 & 89.00 \\ 
\midrule
\multirow{3}{*}{Max}  & - & 77.59 & 77.35 & 70.95 & 82.23 \\
                      & 2        & 81.58 & 73.54 & 72.38 & 83.44 \\
                      & 4        & 78.34 & 79.17 & 76.67 & 84.71 \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/regularization.tex <==
\begin{table*}[htb]
\begin{center}
\setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \begin{tabular}{cccccccccc}
    \hline
         Regularization & Probability & IIIT5K & IC03 & IC13 & SVT & IC15 & SVTP & CUTE80 & Avg\\ \hline
         w/o & - & 51.83 & 59.75 & 59.90 & 37.40 & 31.73 & 28.99 & 32.29 & 43.13\\ 
         w/ & - & 56.30 & 67.70 & 63.25 & 41.27 & 35.05 & 36.90 & 37.15 & 48.23 \\ 
         w/ & 0.5 & 58.03 & 68.17 & 64.83 & 46.21 & 35.34 & 36.12 & 36.46 & 49.31\\ \hline
    \end{tabular}
\caption{\textbf{Ablation of relational regularization module.} ``Regularization" represents that whether or not to add samples for regularization and ``probability" represents the probability of sample regularization. All results are on representation qualities (decoder evaluation accuracy).}
\label{tab:regularization}
\end{center}
\end{table*}

==> tables/representation_quality.tex <==
\begin{table*}[t]
\begin{center}
\setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \begin{tabular}{clcccccccc}
    \hline
        \multirow{2}{*}{Decoder} & \multirow{2}{*}{Method} & \multicolumn{8}{c}{Scene-Text Dataset}\\ 
        \cline{3-10}
        & & IIIT5K & IC03 & IC13 & SVT & IC15 & SVTP & CUTE80 & Avg \\ \hline
        \multirow{7}{*}{CTC} & SeqCLR & 35.70 & 43.60 & 43.50 & - & - & - & - & -\\ 
        ~ & PerSec-CNN & 37.90 & 45.70 & 46.40 & - & - & - & - & -\\ 
        ~ & SeqMoCo & 42.97 & 51.44 & 48.37 & 25.35 & 23.01 & 20.62 & 23.26 & 33.57\\ 
        \cline{2-10}
        ~ & Our method based on SeqMoCo & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\ 
        ~ & w/ reg & 48.43 & 58.94 & 54.98 & 35.09 & 26.43 & 26.82 & 29.17 & 39.98\\ 
        ~ & w/ reg \& hier & 51.90 & 61.36 & 59.01 & 38.79 & 30.62 & 30.08 & 30.21 & 43.14\\ 
        ~ & w/ reg \& hier \& con & 54.83 & 64.82 & 60.89 & 41.58 & 32.6 & 34.26 & 32.64 & 45.95 \\ \hline
        \multirow{7}{*}{Atten} & SeqCLR & 49.20 & 63.90 & 59.30 & - & - & - & - & -\\ 
        ~ & PerSec-CNN & 50.70 & 65.70 & 61.10 & - & - & - & - & -\\ 
        ~ & SeqMoCo & 51.83 & 59.75 & 59.90 & 37.40 & 31.73 & 28.99 & 32.29 & 43.13\\ 
        \cline{2-10}
        ~ & Our method based on SeqMoCo & ~ & ~ & ~ & ~ & ~ & ~ & ~ & ~\\ 
        ~ & w/ reg & 56.30 & 67.70 & 63.25 & 41.27 & 35.05 & 36.9 & 37.15 & 48.23\\ 
        ~ & w/ reg \& hier & 59.03 & 71.51 & 67.29 & 46.37 & 38.32 & 36.90 & 36.81 & 50.89\\ 
        ~ & w/ reg \& hier \& con & 60.83 & 75.20 & 69.66 & 51.78 & 41.12 & 44.03 & 39.93 & 54.65\\ \hline
    \end{tabular}
\caption{\textbf{Representation quality.} Accuracy is used to evaluate the quality of representation from encoder, and we train a decoder with labeled data on top of frozen encoder which was pretrained on unlabeled images. Our method with different modules added is compared with with the previous methods, where "reg" denotes the regularization module, "hier" denotes the hierarchical module and "con" denotes the hierarchical consistency module. }
\label{tab:representation_quality}
\end{center}
\end{table*}

==> tables/semi.tex <==

\begin{table*}[t]
\caption{Main results (\%) on Camelyon16 and TCGA-NSCLC. }
\centering
% \resizebox{1\textwidth}{!}
{\begin{tabular}{clccccccccc} 
\toprule
\multicolumn{3}{c}{\multirow{2}{*}{\diagbox[width=12em]{\textbf{Method}}{\textbf{Performance}}}} & \multicolumn{4}{c}{Camelyon16} & \multicolumn{4}{c}{TCGA-NSCLC} \\ 
\cmidrule(lr){4-7}  
\cmidrule(lr){8-11} 
\multicolumn{3}{r}{} & Precision & Recall  & Accuracy & AUC & Precision & Recall  & Accuracy & AUC\\
\hline
\multirow{12}{*}{\rotatebox{90}{\makecell{ResNet-18 \\ImageNet pretrained}}}
&\multirow{3}{*}{ABMIL}&&86.71&	81.71&	84.50&	84.07& 82.75&	85.84&	81.43&	88.95 \\
&&+IBML                &88.58&	87.14&	88.37&	90.43 & 85.42&	85.17&	85.24&	91.26 \\ 
&&${\Delta}$ & \textcolor{ForestGreen}{+1.87} & \textcolor{ForestGreen}{+5.43} & \textcolor{ForestGreen}{+3.87} & \textcolor{ForestGreen}{+6.36} & \textcolor{ForestGreen}{+2.67}& \textcolor{Red}{-0.67}& 
\textcolor{ForestGreen}{+3.81}
& \textcolor{ForestGreen}{+2.31}\\ \cline{2-11}  
&\multirow{3}{*}{DSMIL}&&84.56&	82.95&	84.50&	87.16& 
80.56&	85.78&	77.62&	86.88\\
&&+IBML 
&90.17&	86.20&	88.37&	87.69& 
81.98&	86.25&	80.00&	87.19 \\ 
&&${\Delta}$ & \textcolor{ForestGreen}{+5.61}& \textcolor{ForestGreen}{+3.25}
& \textcolor{ForestGreen}{+3.87}
& \textcolor{ForestGreen}{+0.53}
& \textcolor{ForestGreen}{+1.42}
& \textcolor{ForestGreen}{+0.47}
& \textcolor{ForestGreen}{+2.38}
& \textcolor{ForestGreen}{+0.31}\\ \cline{2-11}  
&\multirow{3}{*}{TransMIL}&& 85.43	&81.06&	83.72&	81.29 &85.46	&85.31&	85.24&	90.70\\

&&+IBML & 88.39&	84.59&	86.82&	89.49 &85.80	&87.06	&85.24	&92.54\\ 
&&${\Delta}$ & \textcolor{ForestGreen}{+2.96}
& \textcolor{ForestGreen}{+3.53}
& \textcolor{ForestGreen}{+3.10}
& \textcolor{ForestGreen}{+8.20}
& \textcolor{ForestGreen}{+0.34}
& \textcolor{ForestGreen}{+1.75}
& \textcolor{gray}{0.00}
& \textcolor{ForestGreen}{+1.84}
\\ \cline{2-11}  
&\multirow{3}{*}{\makecell{DTFD-MIL \\(MaxS) } }&& 84.85&	80.09&	82.95&	82.77&
82.29&	83.77&	81.90&	88.91\\

&&+IBML & 89.53&	86.51&	88.37&	89.51&
83.25&	82.96&	82.86&	90.50\\

&&${\Delta}$& \textcolor{ForestGreen}{+4.68}
& \textcolor{ForestGreen}{+6.42}
& \textcolor{ForestGreen}{+5.42}
& \textcolor{ForestGreen}{+6.74}
& \textcolor{ForestGreen}{+0.96}
& \textcolor{Red}{-0.81}
& \textcolor{ForestGreen}{+0.96}
& \textcolor{ForestGreen}{+1.59}
\\ 
\cline{2-11}  

% ####################
\hline
\multirow{12}{*}{\rotatebox{90}{\makecell{CTransPath \\ SRCL}}}
&\multirow{3}{*}{ABMIL}&&91.84&	89.09&	90.70&	92.33
&90.76	&90.40&	90.48&	95.87 \\

&&+IBML & 95.29	&92.31&	93.80&	94.36 & 91.92&	91.93&	91.90&	96.91 \\ 
&&${\Delta}$
& \textcolor{ForestGreen}{+3.45}
& \textcolor{ForestGreen}{+3.22}
& \textcolor{ForestGreen}{+3.10}
& \textcolor{ForestGreen}{+2.03}
& \textcolor{ForestGreen}{+1.16}
& \textcolor{ForestGreen}{+1.53}
& \textcolor{ForestGreen}{+1.42}
& \textcolor{ForestGreen}{+1.04}\\ 
\cline{2-11}  
&\multirow{3}{*}{DSMIL}&& 89.24&	88.10&	89.15&	93.26&
92.11&	92.79&	90.95&	97.13\\
&&+IBML & 91.05&	91.30&	91.47&	95.20 
&92.05&	93.82&	91.43&	97.51 \\ 
&&${\Delta}$
& \textcolor{ForestGreen}{+1.81}
& \textcolor{ForestGreen}{+3.20}
& \textcolor{ForestGreen}{+2.31}
& \textcolor{ForestGreen}{+1.94}
& \textcolor{red}{-0.06}
& \textcolor{ForestGreen}{+1.03}
& \textcolor{ForestGreen}{+0.48}
& \textcolor{ForestGreen}{+0.38}
\\ 
\cline{2-11}  
&\multirow{3}{*}{TransMIL}&& 95.83&	93.27&	94.57&	95.88 &93.94	&93.76&	93.81&	95.12\\

&&+IBML &96.48&	95.50&	96.12&	97.00 &93.82	&93.80&	93.81	&96.86\\ 
&&${\Delta}$
& \textcolor{ForestGreen}{+0.35}
& \textcolor{ForestGreen}{+2.33}
& \textcolor{ForestGreen}{+1.55}
& \textcolor{ForestGreen}{+1.12}
& \textcolor{red}{-0.08}
& \textcolor{ForestGreen}{+0.04}
& \textcolor{gray}{0.00}
& \textcolor{ForestGreen}{+1.74}

\\ 
\cline{2-11}  
&\multirow{3}{*}{\makecell{DTFD-MIL \\(MaxS) } }&& 95.87&	94.54&	95.35&	96.18&
90.41&	88.40&	88.57&	94.88\\

&&+IBML & 96.95	&95.19&	96.12&	96.28 
&91.17&	90.89&	90.95&	96.57 \\ 
&&${\Delta}$
& \textcolor{ForestGreen}{+1.08}
& \textcolor{ForestGreen}{+0.65}
& \textcolor{ForestGreen}{+0.77}
& \textcolor{ForestGreen}{+0.10}
& \textcolor{ForestGreen}{+0.76}
& \textcolor{ForestGreen}{+2.49}
& \textcolor{ForestGreen}{+2.38}
& \textcolor{ForestGreen}{+1.69}\\ 
\hline

% #############
\multirow{12}{*}{\rotatebox{90}{\makecell{ViT \\MoCo V3}}}
&\multirow{3}{*}{ABMIL}&&89.95	&83.97&	86.82&	83.94&90.11&89.41&	89.52&	92.85 \\

&&+IBML & 89.01&	86.83&	88.37&	91.38 & 89.79&	89.45&	89.52&	93.29 \\ 
&&${\Delta}$
& \textcolor{red}{-0.94}
& \textcolor{ForestGreen}{+2.86}
& \textcolor{ForestGreen}{+1.55}
& \textcolor{ForestGreen}{+7.44}
& \textcolor{red}{-0.32}
& \textcolor{ForestGreen}{+0.04}
& \textcolor{gray}{0.00}
& \textcolor{ForestGreen}{+0.44}
\\ \cline{2-11}  
&\multirow{3}{*}{DSMIL}&& 86.72&	77.24&	81.40&	82.27& 90.21&	89.93&	90.00&	95.03\\
&&+IBML & 85.08	&78.82&	82.17&	83.77 &91.28&	90.38&	90.48&	95.65\\ 
&&${\Delta}$
& \textcolor{red}{-1.64}
& \textcolor{ForestGreen}{+1.58}
& \textcolor{ForestGreen}{+0.77}
& \textcolor{ForestGreen}{+1.50}
& \textcolor{ForestGreen}{+1.07}
& \textcolor{ForestGreen}{+0.45}
& \textcolor{ForestGreen}{+0.48}
& \textcolor{ForestGreen}{+0.62}
\\ \cline{2-11}  
&\multirow{3}{*}{TransMIL}&&94.70&	92.62&	93.80&	93.93 &95.01	&94.70&	94.76&	96.84 \\

&&+IBML & 94.70&	92.62&	93.80&	95.83 &95.56&	91.89&	91.90&	98.00\\ 
&&${\Delta}$
& \textcolor{gray}{0.00}
& \textcolor{gray}{0.00}
& \textcolor{gray}{0.00}
& \textcolor{ForestGreen}{+1.90}
& \textcolor{ForestGreen}{+0.55}
& \textcolor{red}{-2.81}
& \textcolor{red}{-2.86}
& \textcolor{ForestGreen}{+1.16}
\\ \cline{2-11}  
&\multirow{3}{*}{\makecell{DTFD-MIL \\(MaxS) } }&& 90.71&	88.44&	89.92&	90.96 & 89.45 &	90.89&	89.05&	94.95\\

&&+IBML & 92.65	&92.91&	93.02&	96.35 &91.08	&90.36&	90.48&	96.46\\ 
&&${\Delta}$
& \textcolor{ForestGreen}{+1.94}
& \textcolor{ForestGreen}{+4.47}
& \textcolor{ForestGreen}{+3.10}
& \textcolor{ForestGreen}{+5.39}
& \textcolor{ForestGreen}{+1.63}
& \textcolor{red}{-0.53}
& \textcolor{ForestGreen}{+1.43}
& \textcolor{ForestGreen}{+1.51}
\\  
\bottomrule  
\end{tabular}

\label{tab:c16 tcga}
}
\end{table*}

==> tables/supp_maxmins_c16.tex <==
\begin{table}[t]
\caption{Results on Camelyon16 dataset.}
\label{tab:supp_maxmins_C16}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\makecell{Feature \\Extractor}                   & $K$        & Precision   & Recall   & Accuracy   & AUC  \\ \hline
\multirow{5}{*}{ResNet}  & /  & \color{gray}{84.55} &	\color{gray}{75.62} &	\color{gray}{79.84} &	\color{gray}{79.17} \\
                      & 2  & 87.54&	81.39&	84.5&	85.06 \\
                      & 4        & 79.04&	79.37&	79.84&	84.77 \\
                      & 8        & 86.16&	80.74&	83.72&	85.11 \\
                      & 16        & 81.44 &	81.63&	82.17&	84.44 \\
\midrule

\multirow{5}{*}{CTrans}  & /  & \color{gray}{96.39}	& \color{gray}{94.23}	&\color{gray}{95.35} & \color{gray}{95.15} \\
                      & 2        & 96.95&	95.19&	96.12&	95.75 \\
                      & 4        &96.48 &	95.50&	96.12	&95.95 \\
                      & 8        &96.48	 &95.50	&96.12&	95.95 \\
                      & 16        & 96.48 &	95.50&	96.12&	96.00\\

\midrule
\multirow{5}{*}{ViT}  & /  & \color{gray}{93.84}	& \color{gray}{93.24}	&\color{gray}{93.80} & \color{gray}{94.66} \\
                      & 2        & 95.29&	92.31&	93.80&	94.63 \\
                      & 4        &95.29 &	92.31&	93.80&	94.76 \\
                      & 8        &94.21&	92.93&	93.80&	94.66 \\
                      & 16        & 95.29 &	92.31&	93.80&	94.53\\

\bottomrule
\end{tabular}
}
\end{table}





==> tables/supp_maxmins_tcga.tex <==
\begin{table}[t]
\caption{Results on TCGA-NSCLC dataset.}
\label{tab:supp_maxmins_tcga}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\makecell{Feature \\Extractor}                   & $K$        & Precision   & Recall   & Accuracy   & AUC  \\ \hline
\multirow{5}{*}{ResNet}  & /  & \color{gray}{88.11}	& \color{gray}{88.12}	&\color{gray}{88.10} & \color{gray}{92.36} \\
                      & 2        & 81.84&	91.86&	79.52&	92.95 \\
                      & 4        &86.13 &	85.71&	85.71&	93.41 \\
                      & 8        &87.49 &	85.78&	85.71&	93.61 \\
                      & 16        & 90.01 &	89.99&	90.00&	94.76\\
\midrule

\multirow{5}{*}{CTrans}  & /  & \color{gray}{94.31}	& \color{gray}{94.27}	&\color{gray}{94.29} & \color{gray}{96.74} \\
                      & 2        & 94.31 &	94.27&	94.29&	97.71 \\
                      & 4        &94.72	& 93.80 &	93.81&	97.71 \\
                      & 8        &94.32 &	94.32&	94.29&	97.80 \\
                      & 16        & 94.31 &	94.27&	94.29&	97.68 \\

\midrule
\multirow{5}{*}{ViT}  & /  & \color{gray}{94.29}	& \color{gray}{94.30}	&\color{gray}{94.29} & \color{gray}{98.15} \\
                      & 2        & 94.77&	94.75&	94.76&	98.17 \\
                      & 4        &93.86	 & 94.77&	93.81&	98.19 \\
                      & 8        &94.77	&94.75&	94.76&	98.22 \\
                      & 16        & 94.77&	94.75&	94.76&	98.26\\

\bottomrule
\end{tabular}
}
\end{table}
